A Hierarchical Butterfly LU Preconditioner for Two-Dimensional Electromagnetic Scattering Problems Involving Open Surfaces

This paper introduces a hierarchical interpolative decomposition butterfly-LU factorization (H-IDBF-LU) preconditioner for solving two-dimensional electric-field integral equations (EFIEs) in electromagnetic scattering problems of perfect electrically conducting objects with open surfaces. H-IDBF-LU leverages the interpolative decomposition butterfly factorization (IDBF) to compress dense blocks of the discretized EFIE operator to expedite its application; this compressed operator also serves as an approximate LU factorization of the EFIE operator leading to an efficient preconditioner in iterative solvers. Both the memory requirement and computational cost of the H-IDBF-LU solver scale as $O(N\log^2 N)$ in one iteration; the total number of iterations required for a reasonably good accuracy scales as $O(1)$ to $O(\log^2N)$ in all of our numerical tests. The efficacy and accuracy of the proposed preconditioned iterative solver are demonstrated via its application to a broad range of scatterers involving up to $100$ million unknowns.

==> figure/fig-chpart-ex.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-o}
}
\quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-or}
}
\quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-oc}
}
\quad previous-level blocking \   
\\
\resizebox{0.95cm}{!}{
}\quad \quad \quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-cr}
}
\quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-cc}
}
\quad double-and-halve blocking

\end{minipage}
\caption{An illustration of changing partition. The top-left matrix represents one of blocks in  $S^{4}$ in (\ref{eq:expressUSV4}) or Figure \ref{fig:exlfac}, the top-middle and top-right ones visualize the previous-level partition of rows and columns of the block, respectively. The bottom-left and bottom-right ones visualize the double-and-halve process on the block for next level, as shown in (\ref{eq:exdoubleins}) and (\ref{eq:exS4next}).  }
\label{fig:chpart}
\end{figure}

==> figure/fig-comp-modules/fig-chpart-o.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
      \draw;
\draw[fill=gray] (0,0) rectangle (8,8);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+2);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+1);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+2,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+1,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-complement-1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
      \draw;
\foreach \j in {0,2,...,30}{
    \draw[fill=lightgray] (\j,32) rectangle (\j+2,0);
}
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-complement-2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
      \draw;
\foreach \j in {0,4,...,28}{
    \draw[fill=lightgray] (\j,32) rectangle (\j+4,0);
}
\draw[fill=gray] (0,16) rectangle (32,16);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-complement-4.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
      \draw;
\foreach \j in {0,4,...,28}{
    \draw[fill=lightgray] (32,\j) rectangle (0,\j+4);
}
\draw[fill=gray] (16,0) rectangle (16,32);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-complement-5.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
      \draw;
\foreach \j in {0,2,...,30}{
    \draw[fill=lightgray] (32,\j) rectangle (0,\j+2);
}
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (16,8);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A1U.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (4,8);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A1s.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (16,4);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (8,16);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A2s.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (4,16);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A2v.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (8,4);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-partition-K1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \i in {0,2,...,30}{
   \draw[fill=gray] (0,32-\i) rectangle (32,32-\i-2);
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-partition-K2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \i in {0,2,...,30}{
   \draw[fill=gray] (32-\i,0) rectangle (32-\i-2,32);
}\\
      };
\end{tikzpicture}

==> figure/fig-complement.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{2.5cm}{!}{
\input{figure/fig-comp-modules/fig-complement-1}
}
\quad
\resizebox{2.5cm}{!}{
\input{figure/fig-comp-modules/fig-complement-2}
}
\quad
\resizebox{2.5cm}{!}{
\input{figure/fig-comp-modules/fig-complement-3}
}
\quad
\resizebox{2.5cm}{!}{
\input{figure/fig-comp-modules/fig-complement-4}
}
\quad
\resizebox{2.5cm}{!}{
\input{figure/fig-comp-modules/fig-complement-5}
}
\\
\end{minipage}
\caption{Hierarchical decomposition of the row and column indices
    of a $16\times 16$ matrix. The dyadic trees $T_{X}$ and $T_{\Omega}$ have roots containing $16$ rows and $16$ columns respectively, and their leaves containing only a single row or column. The partition above indicates the complementary low-rank property of the matrix, and assumes that each submatrix is rank-$1$. }
\label{fig:complement}
\end{figure}

==> figure/fig-compression-1D.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-K}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-M}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v}
}\\
\end{minipage}
\caption{The middle level factorization of
    a $64\times 64$ complementary low-rank matrix $K\approx U^3M^3(V^3)^*$
    assuming $r=1$.
    Grey blocks indicate nonzero blocks.
    $U^3$ and $V^3$ are block-diagonal matrices with $8$ blocks.
    The diagonal blocks of $U^3$ and $V^3$ are assembled
    according to Equation \eqref{eq:expression-UV}
    as indicated by black rectangles.
    $M^3$ is a $8\times 8$ block matrix with each block
    $M^3_{i,j}$ itself an $8\times 8$ block matrix
    containing diagonal weights matrix on the $(j,i)$ block.}
\label{fig:compression-1D}
\end{figure}


==> figure/fig-double-block-matrix.tex <==
\begin{figure}[htp]
\begin{minipage}{0.32\textwidth}
\begin{tikzpicture}[scale=0.25]
\draw[draw=black] (0,0) rectangle (16,16);
\draw[draw=black,dashed] (0,8) rectangle (16,12);
\draw[draw=black,dashed] (8,0) rectangle (12,16);
\draw[draw=black] (8,8) rectangle (12,12);
\draw[draw=black,dashed] (9,8) rectangle (10,12);
\draw[draw=black,dashed] (8,9) rectangle (12,10);
\filldraw[fill=lightgray,draw=black] (9,9) rectangle (10,10);
\draw (0,10) node[left=3pt,rectangle,fill=white] {$A$};
\draw (10,16) node[above=3pt,rectangle,fill=white] {$B$};
\draw (8,9.5) node[left=3pt,rectangle,fill=white] {{\tiny $C$}};
\draw (9.5,12) node[above=3pt,rectangle,fill=white] {{\tiny $D$}};
\draw (8,0) node[below=5pt,rectangle,fill=white] {$M_{AB,CD}$};
\end{tikzpicture}
\end{minipage}
\caption{The visualization of the submatrices $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$ in $M_{AB}$. The largest black rectangle represents a matrix $M$ and the smaller one inside $M$ indicates its submatrix $M_{AB}$. From left to right, the light gray boxes inside $M_{AB}$ indicate the submatrices  $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$, respectively.}
\label{fig:double-block-matrix}
\end{figure}
